Digital Security -- A Question of Perspective. A Large-Scale Telephone Survey with Four At-Risk User Groups

This paper investigates the digital security experiences of four at-risk user groups in Germany, including older adults (70+), teenagers (14-17), people with migration backgrounds, and people with low formal education. Using computer-assisted telephone interviews, we sampled 250 participants per group, representative of region, gender, and partly age distributions. We examine their device usage, concerns, prior negative incidents, perceptions of potential attackers, and information sources. Our study provides the first quantitative and nationally representative insights into the digital security experiences of these four at-risk groups in Germany. Our findings show that participants with migration backgrounds used the most devices, sought more security information, and reported more experiences with cybercrime incidents than other groups. Older adults used the fewest devices and were least affected by cybercrimes. All groups relied on friends and family and online news as their primary sources of security information, with little concern about their social circles being potential attackers. We highlight the nuanced differences between the four at-risk groups and compare them to the broader German population when possible. We conclude by presenting recommendations for education, policy, and future research aimed at addressing the digital security needs of these at-risk user groups.

==> Sections/rationale_group-selection.tex <==
Rationale for group selection : why
Older adults
Germany has aging population (like many other western countries) who, amplified by the pandemic, increasingly take up ICT > it is interesting to look at their specicifc experiences and needs, as other works have shown they have specific problems, especially from the age 75+ onwards.

MacDonald \& Forte \cite{mcdonald2022privacy} name “the very old” among groups that are especially vulnerable to privacy risks.

Warford \cite{warford2022sok} also lists them under "at risk".

Wang \cite{wang2017third} calls them "under served", which indicates being more at risk. 

Teenager
In contrast, teenager (age 14-17) in Germany grew up in the era of smartphones, tablets, and wearables, while often being excluded by online panels and legally not able to participate in many studies; little is known on what their concerns and experiences are , what they need to improve – it is important to address and support them while still growing up.
Dunphy et al.~\cite{dunphy2014understanding} argue there is a "need to understand the earliest experiences that individuals have encountering and managing personal privacy and security, but also how these attitudes and practices are shaped across the life course either naturally or through significant life events."

MacDonald \& Forte \cite{mcdonald2022privacy} name “the very young” among groups that are especially vulnerable to privacy risks.

Teenagers are mentioned by Warford et al \cite{warford2022sok} as “at risk group” that can be exposed to disproportionate risks and harms.

Zhao et al. \cite{Zhao2019} found that children do not completely understand certain online privacy risks due to their age and development”, may this be true for teenagers as well?

Wang \cite{wang2017third} calls them "under served", which indicates being more wanat risk. 



Migra
Germany is a land of high immigration, in 2020, 27\% of the German population had a “migration background” \footnote{``Migration background'' is a specific category mostly used in German-speaking countries, referring to residents who either have at least one parent who was born outside of Germany, who themselves migrated to Germany, and/or who hold a foreign citizenship~\cite{eu-06-migration} . While the category is very broad, containing vastly different people in regards to their migration experience, it is likely they have experiences and concerns that differ, are less well reached by specific channels, or may have problems finding relevant information due to language barriers. 

“Immigration status” is mentioned by Sannon et al. \cite{sannon2022privacy} as factor contributing to having unique or increased (privacy related) risks. 

MacDonald \& Forte \cite{mcdonald2022privacy} name being an immigrant among groups that are especially vulnerable to privacy risks.

Warford \cite{warford2022sok} name language barriers as limiting accessibility and contribute to digital safety risks. While we do not know the language levels of this sample precisely, we can assume that this is at least partly true for them (?).

Low Ed
People with Low Education (so far) mostly did not receive education on informatics in school, they are also more like to work in contexts in which they work less with ICT, and are less targeted by awareness campaigns; it is likely they have less access to reliable information sources or have to muster up the resources to do the research on them themselves, therefore it is important to take them into account to better address and support them with fitting materials. 

Sannon et al. \cite{sannon2022privacy} mention “socio-economic status”, which includes Low Ed, as factor contributing to having unique or increased (privacy related) risks.

MacDonald \& Forte \cite{mcdonald2022privacy}d similarly name “socio economic status” as factor contributing to being especially vulnerable to privacy risks.

Warford et al. \cite{warford2022sok} name socio-economic factors as potentially exposing people to more risk. 

Redmiles \cite{redmiles_digital_Divide} found people with low SES to differ from other groups.



Warford \cite{warford2022sok} found that “nearly all at-risk populations had less digital-safety knowledge than they needed to mitigate the risks they faced. While prior work has found that general users tend to have limited digital-safety knowledge [103], this was exacerbated for at-risk users who, by definition, faced serious digital-safety risks and thus usually needed to understand and deploy more robust protections than a typical user.” 
They further argue, that at-risk users are more resource and time constrained to deal with information or to understand security settings. 


==> Tables/Demographics.tex <==
\def\rot{\rotatebox{90}}
\begin{table*}[t]
\small
\caption{Demographics and device usage of the four at-risk groups.}
    \label{tab:demographics}

\tabcolsep=0.5cm
    \begin{tabular}{ll|S[table-format=3]S[table-format=3]|S[table-format=3]S[table-format=3]|S[table-format=3]S[table-format=2]|S[table-format=3]S[table-format=3]}
    \toprule
                                                &   & \multicolumn{2}{c|}{\textbf{Teenagers}}            & \multicolumn{2}{c|}{\textbf{Older Adults}}            & \multicolumn{2}{c|}{\textbf{Migra. Backgr.}}         & \multicolumn{2}{c}{\textbf{Low Education}} \\
                                                &   & \multicolumn{2}{c|}{n=250} & \multicolumn{2}{c|}{n=250}  & \multicolumn{2}{c|}{n=251} & \multicolumn{2}{c}{n=252} \\
                                                &   & \multicolumn{1}{c}{n}      & \multicolumn{1}{c|}{\%}             & \multicolumn{1}{c}{n}   & \multicolumn{1}{c|}{\%}             & \multicolumn{1}{c}{n}   & \multicolumn{1}{c|}{\%} & \multicolumn{1}{c}{n}   & \multicolumn{1}{c}{\%} \\

                                                \cline{1-6} \hline
    \multirow{4}{*}{\rot{\textbf{Age}}}         & \multicolumn{1}{l|}{14-17}            & 250 & 100 & 0   & 0   & 0  & 0 & 0  & 0 \\
                                                & \multicolumn{1}{l|}{17-35}            & 0   & 0   & 0   & 0   & 103  & 41 & 39  & 15 \\
                                                & \multicolumn{1}{l|}{36-50}            & 0   & 0   & 0   & 0   & 63  & 25 & 48  & 19 \\
                                                & \multicolumn{1}{l|}{51-65}              & 0   & 0   & 0 & 0 & 57  & 23 & 68 & 27 \\
                                                & \multicolumn{1}{l|}{66-69}              & 0   & 0   & 0 & 0 & 14  & 5 & 75 & 30 \\
                                                & \multicolumn{1}{l|}{70+}              & 0   & 0   & 250 & 100 & 14  & 5 & 22 & 9 \\
                                                \cline{1-6} \hline
    \multirow{3}{*}{\rot{\textbf{Gender}}}      & \multicolumn{1}{l|}{Male}             & 111 & 44  & 130 & 52           & 128 & 49 & 128 & 51 \\
                                                & \multicolumn{1}{l|}{Female}           & 138 & 55  & 120 & 48           & 123 & 51 & 124 & 49 \\
                                                & \multicolumn{1}{l|}{Non-binary}       & 1   & 1   & 0   & 0           & 0   & 0  & 0   & 0 \\ \cline{1-6} \hline
    \multirow{4}{*}{\rot{\textbf{Region}}}      & \multicolumn{1}{l|}{North}            & 42  & 17  & 39  & 16           & 37  & 15 & 38  & 15 \\
                                                & \multicolumn{1}{l|}{East}             & 51  & 20  & 45  & 18           & 28  & 11 & 24  & 10 \\
                                                & \multicolumn{1}{l|}{South}            & 70  & 28  & 76  & 30           & 82  & 33 & 86  & 34 \\
                                                & \multicolumn{1}{l|}{West}             & 87  & 35  & 90  & 36           & 104 & 41 & 104 & 41 \\ \hline
    \multirow{3}{*}{\rot{\textbf{Education}}}   & Low (ISCED 0-2)                       & 31  & 13                       & 126 & 50                       & 50  & 20                      & 252 & 100 \\
                                                & Medium (ISCED 3-4)                    & 63  & 25                       & 57  & 22                       & 103 & 41                      & 0   & 0 \\
                                                & High (ISCED 4-8)                      & 0   & 0                        & 56  & 22                       & 96  & 38                      & 0   & 0 \\
                                                & Other                                 & 156\protect\footnotemark & 62                       & 11  & 4                        & 3   & 1                       & 0   & 0 \\
                                                \cline{1-6} \hline
    \multirow{6}{*}{\rot{\textbf{Device Usage}}} & \multicolumn{1}{l|}{Smartphone}       & 249 & 99  & 185 & 74  & 244 & 97 & 229 & 91 \\
                                                %& \multicolumn{1}{l|}{Desktop PC}       & 124 & 49  & 119 & 47  & 112 & 44 & 114 & 45 \\
                                                %& \multicolumn{1}{l|}{Laptop}           & 139 & 55  & 126 & 50  & 192 & 76 & 176 & 70 \\
                                                & \multicolumn{1}{l|}{Laptop or Desktop PC}           & 207 & 83  & 194 & 78  & 222 & 88 & 215 & 85 \\
                                                & \multicolumn{1}{l|}{Tablet}           & 138 & 55  & 88  & 35  & 144 & 57 & 121 & 48 \\
                                                & \multicolumn{1}{l|}{Smart Speaker}    & 54  & 21  & 23  & 9   & 72  & 29 & 46  & 18 \\
                                                & \multicolumn{1}{l|}{Wearables}        & 64  & 26  & 28  & 11  & 96  & 38 & 64  & 25 \\
                                                & \multicolumn{1}{l|}{None}        & 18  & 7  & 12  & 5  & 13  & 5 & 17  & 7 \\

    \bottomrule
    \end{tabular}
    
    \end{table*}
    %\footnotemark{}
    %
    %\footnotetext{}{Multiple answers possible.}
   
